PARIC: Probabilistic Attention Regularization for Language Guided Image Classification from Pre-trained Vison Language Models

Language-guided attention frameworks have significantly enhanced both interpretability and performance in image classification; however, the reliance on deterministic embeddings from pre-trained vision-language foundation models to generate reference attention maps frequently overlooks the intrinsic multivaluedness and ill-posed characteristics of cross-modal mappings. To address these limitations, we introduce PARIC, a probabilistic framework for guiding visual attention via language specifications. Our approach enables pre-trained vision-language models to generate probabilistic reference attention maps, which align textual and visual modalities more effectively while incorporating uncertainty estimates, as compared to their deterministic counterparts. Experiments on benchmark test problems demonstrate that PARIC enhances prediction accuracy, mitigates bias, ensures consistent predictions, and improves robustness across various datasets.

==> sec/3_prob_formulation.tex <==
\section{Problem Formulation}
\label{sec:prob_formulation}

This work addresses the challenge of enhancing image classification interpretability and robustness via probabilistic attention regularization. Let \(\mathcal{X} \subseteq \mathbb{R}^{H \times W \times C}\) be the input space of images, where \(H\) and \(W\) denote spatial dimensions and \(C\) the number of channels, and let \(\mathcal{Y}\) be the label set. Consider a neural classifier \(f_{\theta} : \mathcal{X} \to \mathcal{Y}\), parameterized by \(\theta\), which generates spatial attention maps \(A_{\theta}(x) \in \mathbb{R}^{H \times W}\) for each image \(x \in \mathcal{X}\). Our goal is to regularize \(A_{\theta}(x)\) by leveraging a probabilistic attention prior derived from a frozen CLIP encoder, realized through probabilistic adapters akin to ProbVLM. Specifically, each CLIP embedding \(\mathbf{z} = g_{\phi}(x) \in \mathbb{R}^D\) is represented as a Generalized Gaussian Distribution \(p(\mathbf{z};\,\widehat{\mathbf{z}},\alpha,\beta) \propto \exp\bigl(-\,\|\mathbf{z}-\widehat{\mathbf{z}}\|^\beta / \alpha^\beta\bigr)\), where \(\widehat{\mathbf{z}} \in \mathbb{R}^D\) is the mean embedding and \(\alpha,\beta>0\) capture scale and shape; this design reflects both aleatoric (via \(\alpha,\beta\)) and epistemic (via Monte Carlo dropout) uncertainties. The adapters use intra-modal and cross-modal alignment objectives to ensure consistent image-text embeddings. 


Given a learned image embedding distribution \(p_{I}(\mathbf{z})\) with parameters \(\{\widehat{\mathbf{z}},\alpha,\beta\}\), we sample \(K\) embeddings \(\{\mathbf{z}^{(k)}\}_{k=1}^K\) for each \(x\) and fuse these (e.g., by mean or median) into a reference attention map \(A_{\mathrm{ref}}(x) \in \mathbb{R}^{H \times W}\). To direct the classifier’s own attention \(A_{\theta}(x)\) to focus on the same salient regions, we introduce an attention penalty by applying an element-wise product with $(1 - A_{\mathrm{ref}}(x))$, we impose:

\begin{equation}
\label{eq:att-penalty}
\mathcal{L}_{\mathrm{att}}(A_{\theta}(x), A_{\mathrm{ref}}(x)) 
\;=\;
\sum_{i,j}\bigl[(1 - A_{\mathrm{ref}}(x)_{i,j}) \cdot A_{\theta}(x)_{i,j}\bigr],
\end{equation}
which penalizes the classifier for allocating high attention in areas deemed unimportant by \(A_{\mathrm{ref}}(x)\). If the  classification loss of \(f_{\theta}\) is defined via the standard cross-entropy:
\begin{equation}
\label{eq:cls}
\mathcal{L}_{\mathrm{cls}}(f_{\theta}(x),y) 
\;=\; 
-\sum_{c=1}^C \mathbf{1}\{c=y\}\,\log\,p_{\theta}(c\!\mid\!x).
\end{equation}
where $p_{\theta}(c\mid x)$ is the predicted probability for class $c$. The final objective function for EGALS is then formulated as a weighted sum of the classification and the attention regularization loss:

\begin{equation}
\label{eq:total-loss}
\mathcal{L}_{\mathrm{total}}(x,y) 
\;=\;
\mathcal{L}_{\mathrm{cls}}(f_{\theta}(x),y)
\;+\;
\lambda\,\mathcal{L}_{\mathrm{att}}(A_{\theta}(x),A_{\mathrm{ref}}(x)),
\end{equation}
where \(\lambda>0\) balances classification accuracy against attention alignment. By minimizing \(\mathcal{L}_{\mathrm{total}}\), the classifier is guided to concentrate on stable, high-importance regions identified via ProbVLM, resulting in more interpretable and robust predictions.


